Deep Graphic FBSDEs for Opinion Dynamics Stochastic Control

In this paper, we present a scalable deep learning approach to solve opinion dynamics stochastic optimal control problems with mean field term coupling in the dynamics and cost function. Our approach relies on the probabilistic representation of the solution of the Hamilton-Jacobi-Bellman partial differential equation. Grounded on the nonlinear version of the Feynman-Kac lemma, the solutions of the Hamilton-Jacobi-Bellman partial differential equation are linked to the solution of Forward-Backward Stochastic Differential Equations. These equations can be solved numerically using a novel deep neural network with architecture tailored to the problem in consideration. The resulting algorithm is tested on a polarized opinion consensus experiment. The large-scale (10K) agents experiment validates the scalability and generalizability of our algorithm. The proposed framework opens up the possibility for future applications on extremely large-scale problems.

==> Deep Graphical FBSDEs for Opinion Dynamics Control/subtex/math_commands.tex <==
%!TEX root = ../main.tex

%%%%% NEW MATH DEFINITIONS %%%%%

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvX{{\mathbf{X}}}
\def\rvy{{\mathbf{y}}}
\def\rvY{{\mathbf{Y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\Proj}{\mathrm{Proj}}
\newcommand{\Alg}{\mathrm{Alg}}
\newcommand{\vectorize}{\mathrm{vec}}
% \newcommand{\Alg}{\mathrm{Alg}}

% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\let\ab\allowbreak


==> Deep Graphical FBSDEs for Opinion Dynamics Control/subtex/math_util.tex <==
%!TEX root = ../main.tex

\def\comma{{ \text{ ,} }}
\def\period{{ \text{ .} }}

% \def\st{{\quad \text{s.t.} \quad}}
\def\intT{{ \int_{t_0}^{t_1} }}
\def\rintT{{ \int^{t_0}_{t_1} }}
\newcommand{\sdWt}{\circ \mathrm{d}\mathbf{W}_t}
\newcommand{\sdhWt}{\circ \mathrm{d}\overline{\mathbf{W}}_t}
\def\Wt{{ \mathbf{W}_t }}

\def\hvx{{ \bar{\vx} }}
\def\hvu{{ \bar{\vu} }}
\def\hrvx{{ \bar{\rvx} }}
\def\hrvu{{ \bar{\rvu} }}
\def\hrvxt{{ \bar{\rvx}_t }}
\def\hrvut{{ \bar{\rvu}_t }}


\def\hWt{{ \overline{\mathbf{W}}_t }}
\def\drvx{{\delta \rvx}}
\def\drvu{{\delta \rvu}}
\def\drvxt{{\delta \rvx_t}}
\def\drvut{{\delta \rvu_t}}
\def\Lx{{\ell_{\hvx} }}
\def\Lu{{\ell_{\hvu} }}
\def\Lxx{{{\ell}_{\hvx \hvx}}}
\def\Luu{{{\ell}_{\hvu \hvu}}}
\def\Lux{{{\ell}_{\hvu \hvx}}}
\def\Lxu{{{\ell}_{\hvx \hvu}}}
\def\Vx{{V_{\rvx} }}
\def\Vxx{{V_{\rvx\rvx} }}


\def\hS{{\bar{\sigma}}}
\def\hSu{{\bar{\sigma}_\rvu}}
\def\hSx{{\bar{\sigma}_\rvx}}
\def\hST{{\bar{\sigma}^\T}}
\def\hSuT{{\bar{\sigma}^\T_\rvu}}
\def\hSxT{{\bar{\sigma}^\T_\rvx}}
\def\hF{{\bar{F}}}
\def\hFu{{\bar{F}_\rvu}}
\def\hFx{{\bar{F}_\rvx}}
\def\Fu{{{F}_\hvu}}
\def\Fx{{{F}_\hvx}}
\def\FxT{{{F}_\hvx^\T}}
\def\FuT{{{F}_\hvu^\T}}

\def\Gu{{{G}_\rvu}}
\def\Gx{{{G}_\rvx}}
\def\hG{{\bar{G}}}
\def\hGu{{\bar{G}_\rvu}}
\def\hGx{{\bar{G}_\rvx}}
\def\hGT{{\bar{G}^\T}}
\def\hGuT{{\bar{G}^\T_\rvu}}
\def\hGxT{{\bar{G}^\T_\rvx}}

\def\Su{{{\sigma}_\rvu}}
\def\Sx{{{\sigma}_\rvx}}
\def\SxT{{{\sigma}_\rvx^\T}}
\def\SuT{{{\sigma}_\rvu^\T}}

\def\QxT{{Q^\T_{\hvx}}}
\def\QuT{{Q^\T_{\hvu}}}
\def\Qx{{Q_{\hvx}}}
\def\Qu{{Q_{\hvu}}}
\def\Qxu{{Q_{\hvx \hvu}}}
\def\Qxx{{Q_{\hvx \hvx}}}
\def\Quu{{Q_{\hvu \hvu}}}
\def\Qux{{Q_{\hvu \hvx}}}
\def\srd{{\circ\rd}}
\newcommand{\sfracdiff}[2]{\frac{\srd #1}{\rd  #2}}
\def\htheta{{\hat{\theta}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%
% DDP
%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\norm}[1]{\left\lVert#1\right\rVert}


\def\ttranspose{{t \text{ } \transpose}}
\def\vxr{{\vx_r}}
% \def\dvxr{{\delta \vx_r}}

\def\kt{{\vk}}
\def\Kt{{\mK}}
\def\Gt{{\mathbf{G}_t}}

\def\KtT{{\mathbf{K}_t^\transpose}}
\def\GtT{{\mathbf{G}_t^\transpose}}


\def\It{{\mathbf{I}_t}}
\def\Lt{{\mathbf{L}_t}}
\def\Ht{{\mathbf{H}_t}}

\def\kut{{\tilde{\mathbf{k}}_t}}
\def\Kut{{\tilde{\mathbf{K}}_t}}
\def\Gut{{\tilde{\mathbf{G}}_t}}

\def\Ivt{{\tilde{\mathbf{I}}_t}}
\def\Lvt{{\tilde{\mathbf{L}}_t}}
\def\Hvt{{\tilde{\mathbf{H}}_t}}

\def\QuuC{{\tilde{Q}_{\vu \vu}}}
\def\QvvC{{\tilde{Q}_{\vv \vv}}}
\def\QuutC{{\tilde{Q}^t_{\vu \vu}}}
\def\QvvtC{{\tilde{Q}^t_{\vv \vv}}}
\def\QuuCInv{{\tilde{Q}^{-1}_{\vu \vu}}}
\def\QvvCInv{{\tilde{Q}^{-1}_{\vv \vv}}}
\def\QA{{Q_{\vu \vx_r}}}
\def\QB{{Q_{\vv \vx}}}
\def\QAt{{Q^t_{\vu \vx_r}}}
\def\QBt{{Q^t_{\vv \vx}}}

\def\Axx{{\E[\vx_{\vu}\vx_{\vu}^\transpose]}}
\def\Axy{{\E[\vx_{\vu}\vx_{\vv}^\transpose]}}
\def\Ayy{{\E[\vx_{\vv}\vx_{\vv}^\transpose]}}
\def\Ayx{{\E[\vx_{\vv}\vx_{\vu}^\transpose]}}
\def\Bxx{{\E[\vg_{\vu}\vg_{\vu}^\transpose]}}
\def\Bxy{{\E[\vg_{\vu}\vg_{\vv}^\transpose]}}
\def\Byy{{\E[\vg_{\vv}\vg_{\vv}^\transpose]}}
\def\Byx{{\E[\vg_{\vv}\vg_{\vu}^\transpose]}}

\def\Auu{{A_{\vu\vu}}}
\def\Auv{{A_{\vu\vv}}}
\def\Avu{{A_{\vv\vu}}}
\def\Avv{{A_{\vv\vv}}}
\def\Buu{{B_{\vu\vu}}}
\def\Buv{{B_{\vu\vv}}}
\def\Bvu{{B_{\vv\vu}}}
\def\Bvv{{B_{\vv\vv}}}
\def\AuvT{{A^\transpose_{\vu\vv}}}
\def\BuvT{{B^\transpose_{\vu\vv}}}
\def\AvuT{{A^\transpose_{\vv\vu}}}
\def\BvuT{{B^\transpose_{\vv\vu}}}
\def\AuuInv{{A^{-1}_{\vu\vu}}}
\def\AvvInv{{A^{-1}_{\vv\vv}}}
\def\BuuInv{{B^{-1}_{\vu\vu}}}
\def\BvvInv{{B^{-1}_{\vv\vv}}}
\def\AuuCInv{{\tilde{A}^{-1}_{\vu\vu}}}
\def\BuuCInv{{\tilde{B}^{-1}_{\vu\vu}}}
\def\AvvCInv{{\tilde{A}^{-1}_{\vv\vv}}}
\def\BvvCInv{{\tilde{B}^{-1}_{\vv\vv}}}
\def\AvvInvT{{A^{-\transpose}_{\vv\vv}}}
\def\AuuCInvT{{\tilde{A}^{-\transpose}_{\vu\vu}}}

% \def\Dxu{{\nabla_{\vu \vx}}}
% \def\llxu{{{\ell}(\vx^{(i)},\vu)}}
% \def\ffxu{{{f}(\vx^{(i)},\vu)}}
% \def\Lx{{\mathbf{L}_{\mX}}}
% \def\Lu{{\mathbf{L}_{\vu}}}
% \def\Lxx{{\mathbf{L}_{\mX \mX}}}
% \def\Luu{{\mathbf{L}_{\vu \vu}}}
% \def\Lux{{\mathbf{L}_{\vu \mX}}}
% \def\Fu{{\mathbf{F}_\vu}}
% \def\Fx{{\mathbf{F}_\mX}}
% \def\FxT{{\mathbf{F}_\mX^\transpose}}
% \def\FuT{{\mathbf{F}_\vu^\transpose}}
% \def\Fxx{{\mathbf{F}_{\mX \mX}}}
% \def\Fuu{{\mathbf{F}_{\vu \vu}}}
% \def\Fux{{\mathbf{F}_{\vu \mX}}}
\def\VxN{{\mathbf{V}_\mX^T}}
\def\VxxN{{\mathbf{V}_{\mX\mX}^T}}
% \def\QQX{{\mathbf{Q}_\mX}}
% \def\QQu{{\mathbf{Q}_\vu}}
% \def\QQXX{{\mathbf{Q}_{\mX\mX}}}
% \def\QQuu{{\mathbf{Q}_{\vu\vu}}}
% \def\QQuX{{\mathbf{Q}_{\vu\mX}}}
% \def\QQuuInv{{\mathbf{Q}^{-1}_{\vu\vu}}}
% \def\QQuuInvApprox{{\mathbf{\widetilde{Q}}^{-1}_{\vu\vu}}}
% \def\QQuXT{{\mathbf{Q}^\transpose_{\vu\mX}}}
% \def\VXNxt{{\mathbf{V}^\prime_{\mX}}}
% \def\VXXNxt{{\mathbf{V}^\prime_{\mX\mX}}}

\def\VX{{\mathbf{V}_{\mX}}}
\def\VXX{{\mathbf{V}_{\mX\mX}}}

\def\QQXt{{\mathbf{Q}^t_\mX}}
\def\QQut{{\mathbf{Q}^t_\vu}}
\def\QQXXt{{\mathbf{Q}^t_{\mX\mX}}}
\def\QQuut{{\mathbf{Q}^t_{\vu\vu}}}
\def\QQuXt{{\mathbf{Q}^t_{\vu\mX}}}
\def\QQuuInvt{{[\mathbf{Q}^{t}_{\vu\vu}]^{-1}}}
\def\VXt{{\mathbf{V}^t_{\mX}}}
\def\VXXt{{\mathbf{V}^t_{\mX\mX}}}


\def\xxi{{\vx_t^{(i)}}}

\def\dvx{{\delta\vx}}
\def\dvu{{\delta\vu}}
\def\dvv{{\delta\vv}}
\def\vxTraj{{\bar{\vx}}}
\def\vuTraj{{\bar{\vu}}}

\def\Inv{{-1}}
% \def\Inv{{\dagger}}

\def\ConvT{{\text{ } \hat{*} \text{ }}}
% \def\ConvT{{*^\transpose}}
\def\eqConv{{\text{ }\text{ } \stackrel{\mathclap{\tiny\mbox{conv}}}{=}\text{ }\text{ } }}

\def\Vh{{V_{\vh}}}
\def\Vht{{V^{t}_{\vh}}}
\def\Vhht{{V^{t}_{\vh\vh}}}
% \def\Vxt{{V^{t+1}_{\vx}}}
% \def\Vxxt{{V^{t+1}_{\vx\vx}}}
% \def\Vx{{V_{\vx^{\prime}}^{\prime}}}
% \def\Vxx{{V_{\vx^{\prime} \vx^{\prime}}^{\prime}}}

% \def\Qxt{{Q^t_{\vx}}}
% \def\Qut{{Q^t_{\vu}}}
% \def\Qxxt{{Q^t_{\vx \vx}}}
% \def\Quxt{{Q^t_{\vu \vx}}}
% \def\Qxut{{Q^t_{\vx \vu}}}
% \def\Quut{{Q^t_{\vu \vu}}}
% \def\Qx{{Q_{\vx}}}
% \def\Qu{{Q_{\vu}}}
% \def\Qxx{{Q_{\vx \vx}}}
% \def\Quu{{Q_{\vu \vu}}}
% \def\QuuInv{{Q^{-1}_{\vu \vu}}}
% \def\QuuInvt{{({Q^{t}_{\vu \vu})}^{-1}}}
% \def\Qux{{Q_{\vu \vx}}}
% \def\Qxu{{Q_{\vx \vu}}}

% \def\Qvt{{Q^t_{\vv}}}
% \def\Qvxt{{Q^t_{\vv \vx}}}
% \def\Qvyt{{Q^t_{\vv \vx_r}}}
% \def\Qxvt{{Q^t_{\vx \vv}}}
% \def\Qvvt{{Q^t_{\vv \vv}}}
% \def\Quvt{{Q^t_{\vu \vv}}}
% \def\Qvut{{Q^t_{\vv \vu}}}
% \def\Qv{{Q_{\vv}}}
% \def\Qvv{{Q_{\vv \vv}}}
% \def\QvvInv{{Q^{-1}_{\vv \vv}}}
% \def\QvvInvt{{({Q^{t}_{\vv \vv})}^{-1}}}
% \def\Qvx{{Q_{\vv \vx}}}
% \def\Qxv{{Q_{\vx \vv}}}
% \def\Quv{{Q_{\vu \vv}}}
% \def\Qvu{{Q_{\vv \vu}}}
% \def\Qvy{{Q_{\vv \vx_r}}}
% \def\QvuT{{Q^\transpose_{\vv \vu}}}

\def\fx{{{f}_{\vx}}}
\def\fu{{{f}_{\vu}}}
\def\fxt{{{f}^t_{\vx}}}
\def\fut{{{f}^t_{\vu}}}
\def\fuT{{{f}_{\vu}^\transpose}}
\def\fxT{{{f}_{\vx}^\transpose}}
\def\futT{{{{f}^t_{\vu}}^\transpose}}
\def\fxtT{{{{f}^t_{\vx}}^\transpose}}
\def\fxx{{{f}_{\vx \vx}}}
\def\fuu{{{f}_{\vu \vu}}}
\def\fux{{{f}_{\vu \vx}}}
\def\fxu{{{f}_{\vx \vu}}}
\def\fxxt{{{f}^t_{\vx \vx}}}
\def\fuut{{{f}^t_{\vu \vu}}}
\def\fuxt{{{f}^t_{\vu \vx}}}
\def\fxut{{{f}^t_{\vx \vu}}}

\def\gutT{{{g}^{t \text{ }\transpose}_{\vu}}}
\def\gxtT{{{g}^{t \text{ }\transpose}_{\vx}}}
\def\gut{{{g}^{t}_{\vu}}}
\def\gxt{{{g}^{t}_{\vx}}}
\def\sht{{{\sigma}^{t}_{\vh}}}
\def\shtT{{{\sigma}^{t \text{ }\transpose}_{\vh}}}

\def\lxt{{{\ell}^t_{\vx}}}
\def\lut{{{\ell}^t_{\vu}}}
\def\lxxt{{{\ell}^t_{\vx \vx}}}
\def\luut{{{\ell}^t_{\vu \vu}}}
\def\luxt{{{\ell}^t_{\vu \vx}}}
\def\lxut{{{\ell}^t_{\vx \vu}}}


\def\lx{{{\ell}_{\vx}}}
\def\lu{{{\ell}_{\vu}}}
\def\lxx{{{\ell}_{\vx \vx}}}
\def\luu{{{\ell}_{\vu \vu}}}
\def\lux{{{\ell}_{\vu \vx}}}
\def\lxu{{{\ell}_{\vx \vu}}}

\def\gx{{{g}_{\vx}}}
\def\gu{{{g}_{\vu}}}
\def\gxx{{{g}_{\vx \vx}}}
\def\guu{{{g}_{\vu \vu}}}
\def\gux{{{g}_{\vu \vx}}}
\def\gxu{{{g}_{\vx \vu}}}

\def\gxxt{{{g}^t_{\vx \vx}}}
\def\guut{{{g}^t_{\vu \vu}}}
\def\guxt{{{g}^t_{\vu \vx}}}
\def\gxut{{{g}^t_{\vx \vu}}}


\def\Dxu{{\nabla_{\vu \vx}}}
\def\llxu{{{\ell}(\vx^{(i)},\vu)}}
\def\ffxu{{{f}(\vx^{(i)},\vu)}}
% \def\Lx{{\mathbf{L}_{\mX}^t}}
% \def\Lu{{\mathbf{L}_{\vu}^t}}
% \def\Lxx{{\mathbf{L}^t_{\mX \mX}}}
% \def\Luu{{\mathbf{L}^t_{\vu \vu}}}
% \def\Lux{{\mathbf{L}^t_{\vu \mX}}}

% \def\Fu{{\mathbf{F}^t_\vu}}
% \def\Fx{{\mathbf{F}^t_\mX}}
% \def\FxT{{{\mathbf{F}^{t\transpose}_\mX}}}
% \def\FuT{{{\mathbf{F}^{t\transpose}_\vu}}}
% \def\Fxx{{\mathbf{F}^t_{\mX \mX}}}
% \def\Fuu{{\mathbf{F}^t_{\vu \vu}}}
% \def\Fux{{\mathbf{F}^t_{\vu \mX}}}

% \def\Gu{{\mathbf{G}^t_\vu}}
% \def\Gx{{\mathbf{G}^t_\mX}}
% \def\GxT{{{\mathbf{G}^{t\transpose}_\mX}}}
% \def\GuT{{{\mathbf{G}^{t\transpose}_\vu}}}
% \def\Gxx{{\mathbf{G}^t_{\mX \mX}}}
% \def\Guu{{\mathbf{G}^t_{\vu \vu}}}
% \def\Gux{{\mathbf{G}^t_{\vu \mX}}}

\def\VH{{\mathbf{V}^t_{\mH}}}
\def\VhN{{\mathbf{V}_\mH^T}}
\def\VhhN{{\mathbf{V}_{\mH\mH}^T}}
\def\VHNxt{{\mathbf{V}^\prime_{\mH^\prime}}}
\def\VHHNxt{{\mathbf{V}^t_{\mH\mH}}}


% \def\VxN{{\mathbf{V}_\mX^T}}
% \def\VxxN{{\mathbf{V}_{\mX\mX}^T}}
\def\QQX{{\mathbf{Q}_\mX^t}}
\def\QQu{{\mathbf{Q}_\vu^t}}
\def\QQXX{{\mathbf{Q}^t_{\mX\mX}}}
\def\QQuu{{\mathbf{Q}^t_{\vu\vu}}}
\def\QQuX{{\mathbf{Q}^t_{\vu\mX}}}
\def\QQuuInv{{\mathbf{Q}^{-1}_{\vu\vu}}}
\def\QQuuInvApprox{{\mathbf{\widetilde{Q}}^{-1}_{\vu\vu}}}
\def\QQuXT{{{\mathbf{Q}^{t\transpose}_{\vu\mX}}}}
\def\VXNxt{{\mathbf{V}^\prime_{\mX^\prime}}}
\def\VXXNxt{{\mathbf{V}^\prime_{\mX^\prime\mX^\prime}}}

\def\QQXprevT{{\mathbf{Q}_\mX^{T-1}}}
\def\QQuprevT{{\mathbf{Q}_\vu^{T-1}}}
\def\QQXXprevT{{\mathbf{Q}^{T-1}_{\mX\mX}}}
\def\QQuuprevT{{\mathbf{Q}^{T-1}_{\vu\vu}}}
\def\QQuXprevT{{\mathbf{Q}^{T-1}_{\vu\mX}}}

\def\VX{{\mathbf{V}_{\mX}}}
\def\VXX{{\mathbf{V}_{\mX\mX}}}

\def\QQXt{{\mathbf{Q}^t_\mX}}
\def\QQut{{\mathbf{Q}^t_\vu}}
\def\QQXXt{{\mathbf{Q}^t_{\mX\mX}}}
\def\QQuut{{\mathbf{Q}^t_{\vu\vu}}}
\def\QQuXt{{\mathbf{Q}^t_{\vu\mX}}}
\def\QQuuInvt{{(\mathbf{Q}^{t}_{\vu\vu})^{-1}}}
\def\VXt{{\mathbf{V}^t_{\mX}}}
\def\VXXt{{\mathbf{V}^t_{\mX\mX}}}

\def\idxFu{{(B_{n_{t^\prime}}^{(i)},:)}}
\def\idxFuu{{(B_{n_{t^\prime}}^{(i)},:,:)}}
\def\idxFx{{(B_{n_{t^\prime}}^{(i)},B_{n_{t}}^{(j)})}}
\def\idxFux{{(B_{n_{t^\prime}}^{(i)},:,B_{n_{t}}^{(j)})}}
\def\idxFxx{{(B_{n_{t^\prime}}^{(i)},B_{n_{t}}^{(j)},B_{n_{t}}^{(k)})}}

%%%%%%%%%%%%%%%%%%%%%%%%%%
% Mean field optimal control
%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\cspace{{\mathbb{R}^{m}}}
\def\Cspace{{\mathbb{R}^{\bar{m}}}}
\def\Xspace{{\mathbb{R}^{n}}}
\def\xyspace{{\mathbb{R}^{n+d}}}
% \def\Cspace{{\mathbb{R}^{mT}}}
\def\yspace{{\mathbb{R}^{d}}}
\def\expdnn{{\mathbb{E}_{\substack{ (\rvx_t, \rvy) \sim \mu_t \\ \text{subject to (\ref{eq:fc-dnn-dynamics})}}}}}% expectation

\def\transpose{{\mathsf{T}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%
% SGD formulation
%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\gradsampleeq{{
    \nabla_\vtheta l ( f ( \rvx^{(i)}, \vtheta ), \rvy^{(i)} )
}}
\def\gradsample{{ g^{i}(\vtheta) }}
\def\gradmb{{ g^{mb}(\vtheta) }}
\def\gradfull{{ g^{}(\vtheta) }}
\def\gradmbt{{   g^{mb}(\vtheta_{t}) }}
\def\gradfullt{{ g^{}(\vtheta_{t}) }}
\def\diffusionmatrixx{{ \mathbf{\Sigma}_{\mathcal{D}} }}
\def\diffusionmatrix{{ \mathbf{\Sigma}_{\mathcal{D}}(\vtheta) }}
\def\diffusionmatrixt{{ \mathbf{\Sigma}_{\mathcal{D}}(\vtheta_{t}) }}
% \def\diffusionmatrixthaft{{  \mathbf{\Sigma}^{1/2}_{        \mathcal{D}}(\vtheta_{t}) }}
\def\diffusionmatrixthaft{{ \mathbf{\Sigma}^{\frac{1}{2}}_{\mathcal{D}}(\vtheta_{t}) }}
\def\diffusionmatrixthaftt{{ \mathbf{\Sigma}^{\frac{1}{2}}_{\mathcal{D}} }}
% \def\diffusionmatrixthafttt{{ \tilde{\mathbf{\Sigma}}^{\frac{1}{2}}_{\mathcal{D}}(\vtheta_{t}) }}
\def\diffusionmatrixthafttt{{ \tilde{\mathbf{\Sigma}}^{\frac{1}{2}}_{\mathcal{D}} }}
\def\diffusionmatrixttt{{ \tilde{\mathbf{\Sigma}}_{\mathcal{D}} }}
\def\diffusionmatrixbatch{{ \tilde{\mathbf{\Sigma}}_{\mathcal{B}} }}
%
% \def\abs#1{ \mid {#1} \mid }
\def\absB{{ \mid \mathcal{B} \mid }}
\def\absD{{ \mid \mathcal{D} \mid }}
%
\def\drift{{ b(\vtheta_{t}) }}
\def\diffusion{{ \sigma(\vtheta_{t}) }}
\def\dt{{ \mathrm{d} t }}
\def\ds{{ \mathrm{d} s }}
\def\dWt{{ \mathrm{d} \mathbf{W}_t }}
\def\dLat{{ \mathrm{d} L_t^{\alpha} }}
\def\tt{{ \vtheta_{t} }}

\def\pss{{ \rho^{\mathrm{ss}} }}
\def\psss{{ \rho^{\mathrm{ss}}(\vtheta) }}

\def\Dk{{ \mathrm{D}^k }}
\def\gmbupdate{{ \vtheta^{\prime} - \eta g^{mb}(\vtheta^{\prime}) }}
\def\gmbupdatee{{ \vtheta - \eta g^{mb}(\vtheta) }}
% \def\deltaa{{ \delta\left( \vtheta - \left(\gmbupdate\right) \right) }}
\def\deltaa{{ \delta\left\{ \vtheta - \left[\gmbupdate\right] \right\} }}
\def\thprime{{ \vtheta^{\prime} }}
\def\dthprime{{ \mathrm{d} \thprime }}
\def\dth{{ \mathrm{d} \vtheta }}
\def\expB{{   \mathbb{E}_{\mathcal{B}} }}
\def\expPss{{ \mathbb{E}_{\pss} }}
% \def\smallint{\begingroup\textstyle \int\endgroup}
\def\smallint{ \int}
\def\smallsum{\begingroup\textstyle \sum \endgroup}

\def\expBof#1{ \expB \left[ {#1} \right]}
\def\expPssof#1{ \expPss \left[ {#1} \right]}
\def\Phigmd{{ \Phi \left(\gmbupdatee\right) }}

\def\itoarg{{\left( X_t, t \right) }}


%%%%%%%%%%%%%%%%%%%%%%%%%%
% Beyong Supervised Learning
%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\thetap{{ \vtheta^{\prime} }}
\def\LocalEntropy{{ - \log \int_{\thetap \in \cspace} \exp (-\Phi (\thetap)-\frac{\gamma}{2}\|\vtheta-\thetap\|_{2}^{2}) \mathrm{d} \thetap }}
\def\LocalEntropyy{{ - \log \int_{\thetap} \exp \left(-\Phi (\thetap)-\frac{\gamma}{2}\|\vtheta-\thetap\|_{2}^{2}\right) \mathrm{d} \thetap }}
\def\ExpOf#1{ \mathbb{E} \left[ {#1} \right]}
\def\ExpOfXi#1{ \mathbb{E}_\xi \left[ {#1} \right]}
\def\ExpOfGibbs#1{ \mathbb{E}_{ \mathcal{P}_\gamma} \left[ {#1} \right]}
\def\fracK {{\frac{1}{k}}}

\def\metanext{{ \vtheta_{\text{adapt}}^{n+1} }}
\def\metacurr{{ \vtheta_{\text{adapt}}^{n}   }}


%Capital caligraphic letters
\def\calA{{\cal A}}
\def\calB{{\cal B}}
\def\calC{{\cal C}}
\def\calD{{\cal D}}
\def\calE{{\cal E}}
\def\calF{{\cal F}}
\def\calG{{\cal G}}
\def\calH{{\cal H}}
\def\calI{{\cal I}}
\def\calJ{{\cal J}}
\def\calK{{\cal K}}
\def\calL{{\cal L}}
\def\calM{{\cal M}}
\def\calN{{\cal N}}
\def\calO{{\cal O}}
\def\calP{{\cal P}}
\def\calQ{{\cal Q}}
\def\calR{{\cal R}}
\def\calS{{\cal S}}
\def\calT{{\cal T}}
\def\calU{{\cal U}}
\def\calV{{\cal V}}
\def\calW{{\cal W}}
\def\calX{{\cal X}}
\def\calY{{\cal Y}}
\def\calZ{{\cal Z}}

\newcommand{\nicefracpartial}[2]{\nicefrac{\partial #1}{\partial  #2}}
\newcommand{\nicefracdiff}[2]{\nicefrac{\rd #1}{\rd  #2}}
\newcommand{\fracpartial}[2]{\frac{\partial #1}{\partial  #2}}
\newcommand{\fracdiff}[2]{\frac{\rd #1}{\rd  #2}}
\newcommand{\br}[1]{\left[#1\right]}
\newcommand{\pr}[1]{\left(#1\right)}
\newcommand{\T}{\mathsf{T}}
\newcommand*\bvec[1]{\begin{bmatrix}#1\end{bmatrix}}
\newcommand{\bmat}[4]{\begin{bmatrix} #1 & #2 \\ #3 & #4\end{bmatrix}}
\def\vec{{\mathrm{vec}}}


==> Deep Graphical FBSDEs for Opinion Dynamics Control/subtex/package.tex <==
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\T}{\mathsf{T}}
% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvX{{\mathbf{X}}}
\def\rvy{{\mathbf{y}}}
\def\rvY{{\mathbf{Y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

==> subtex/math_commands.tex <==
%!TEX root = ../main.tex

%%%%% NEW MATH DEFINITIONS %%%%%

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvX{{\mathbf{X}}}
\def\rvy{{\mathbf{y}}}
\def\rvY{{\mathbf{Y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\Proj}{\mathrm{Proj}}
\newcommand{\Alg}{\mathrm{Alg}}
\newcommand{\vectorize}{\mathrm{vec}}
% \newcommand{\Alg}{\mathrm{Alg}}

% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\let\ab\allowbreak


==> subtex/math_util.tex <==
%!TEX root = ../main.tex

\def\comma{{ \text{ ,} }}
\def\period{{ \text{ .} }}

% \def\st{{\quad \text{s.t.} \quad}}
\def\intT{{ \int_{t_0}^{t_1} }}
\def\rintT{{ \int^{t_0}_{t_1} }}
\newcommand{\sdWt}{\circ \mathrm{d}\mathbf{W}_t}
\newcommand{\sdhWt}{\circ \mathrm{d}\overline{\mathbf{W}}_t}
\def\Wt{{ \mathbf{W}_t }}

\def\hvx{{ \bar{\vx} }}
\def\hvu{{ \bar{\vu} }}
\def\hrvx{{ \bar{\rvx} }}
\def\hrvu{{ \bar{\rvu} }}
\def\hrvxt{{ \bar{\rvx}_t }}
\def\hrvut{{ \bar{\rvu}_t }}


\def\hWt{{ \overline{\mathbf{W}}_t }}
\def\drvx{{\delta \rvx}}
\def\drvu{{\delta \rvu}}
\def\drvxt{{\delta \rvx_t}}
\def\drvut{{\delta \rvu_t}}
\def\Lx{{\ell_{\hvx} }}
\def\Lu{{\ell_{\hvu} }}
\def\Lxx{{{\ell}_{\hvx \hvx}}}
\def\Luu{{{\ell}_{\hvu \hvu}}}
\def\Lux{{{\ell}_{\hvu \hvx}}}
\def\Lxu{{{\ell}_{\hvx \hvu}}}
\def\Vx{{V_{\rvx} }}
\def\Vxx{{V_{\rvx\rvx} }}


\def\hS{{\bar{\sigma}}}
\def\hSu{{\bar{\sigma}_\rvu}}
\def\hSx{{\bar{\sigma}_\rvx}}
\def\hST{{\bar{\sigma}^\T}}
\def\hSuT{{\bar{\sigma}^\T_\rvu}}
\def\hSxT{{\bar{\sigma}^\T_\rvx}}
\def\hF{{\bar{F}}}
\def\hFu{{\bar{F}_\rvu}}
\def\hFx{{\bar{F}_\rvx}}
\def\Fu{{{F}_\hvu}}
\def\Fx{{{F}_\hvx}}
\def\FxT{{{F}_\hvx^\T}}
\def\FuT{{{F}_\hvu^\T}}

\def\Gu{{{G}_\rvu}}
\def\Gx{{{G}_\rvx}}
\def\hG{{\bar{G}}}
\def\hGu{{\bar{G}_\rvu}}
\def\hGx{{\bar{G}_\rvx}}
\def\hGT{{\bar{G}^\T}}
\def\hGuT{{\bar{G}^\T_\rvu}}
\def\hGxT{{\bar{G}^\T_\rvx}}

\def\Su{{{\sigma}_\rvu}}
\def\Sx{{{\sigma}_\rvx}}
\def\SxT{{{\sigma}_\rvx^\T}}
\def\SuT{{{\sigma}_\rvu^\T}}

\def\QxT{{Q^\T_{\hvx}}}
\def\QuT{{Q^\T_{\hvu}}}
\def\Qx{{Q_{\hvx}}}
\def\Qu{{Q_{\hvu}}}
\def\Qxu{{Q_{\hvx \hvu}}}
\def\Qxx{{Q_{\hvx \hvx}}}
\def\Quu{{Q_{\hvu \hvu}}}
\def\Qux{{Q_{\hvu \hvx}}}
\def\srd{{\circ\rd}}
\newcommand{\sfracdiff}[2]{\frac{\srd #1}{\rd  #2}}
\def\htheta{{\hat{\theta}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%
% DDP
%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\norm}[1]{\left\lVert#1\right\rVert}


\def\ttranspose{{t \text{ } \transpose}}
\def\vxr{{\vx_r}}
% \def\dvxr{{\delta \vx_r}}

\def\kt{{\vk}}
\def\Kt{{\mK}}
\def\Gt{{\mathbf{G}_t}}

\def\KtT{{\mathbf{K}_t^\transpose}}
\def\GtT{{\mathbf{G}_t^\transpose}}


\def\It{{\mathbf{I}_t}}
\def\Lt{{\mathbf{L}_t}}
\def\Ht{{\mathbf{H}_t}}

\def\kut{{\tilde{\mathbf{k}}_t}}
\def\Kut{{\tilde{\mathbf{K}}_t}}
\def\Gut{{\tilde{\mathbf{G}}_t}}

\def\Ivt{{\tilde{\mathbf{I}}_t}}
\def\Lvt{{\tilde{\mathbf{L}}_t}}
\def\Hvt{{\tilde{\mathbf{H}}_t}}

\def\QuuC{{\tilde{Q}_{\vu \vu}}}
\def\QvvC{{\tilde{Q}_{\vv \vv}}}
\def\QuutC{{\tilde{Q}^t_{\vu \vu}}}
\def\QvvtC{{\tilde{Q}^t_{\vv \vv}}}
\def\QuuCInv{{\tilde{Q}^{-1}_{\vu \vu}}}
\def\QvvCInv{{\tilde{Q}^{-1}_{\vv \vv}}}
\def\QA{{Q_{\vu \vx_r}}}
\def\QB{{Q_{\vv \vx}}}
\def\QAt{{Q^t_{\vu \vx_r}}}
\def\QBt{{Q^t_{\vv \vx}}}

\def\Axx{{\E[\vx_{\vu}\vx_{\vu}^\transpose]}}
\def\Axy{{\E[\vx_{\vu}\vx_{\vv}^\transpose]}}
\def\Ayy{{\E[\vx_{\vv}\vx_{\vv}^\transpose]}}
\def\Ayx{{\E[\vx_{\vv}\vx_{\vu}^\transpose]}}
\def\Bxx{{\E[\vg_{\vu}\vg_{\vu}^\transpose]}}
\def\Bxy{{\E[\vg_{\vu}\vg_{\vv}^\transpose]}}
\def\Byy{{\E[\vg_{\vv}\vg_{\vv}^\transpose]}}
\def\Byx{{\E[\vg_{\vv}\vg_{\vu}^\transpose]}}

\def\Auu{{A_{\vu\vu}}}
\def\Auv{{A_{\vu\vv}}}
\def\Avu{{A_{\vv\vu}}}
\def\Avv{{A_{\vv\vv}}}
\def\Buu{{B_{\vu\vu}}}
\def\Buv{{B_{\vu\vv}}}
\def\Bvu{{B_{\vv\vu}}}
\def\Bvv{{B_{\vv\vv}}}
\def\AuvT{{A^\transpose_{\vu\vv}}}
\def\BuvT{{B^\transpose_{\vu\vv}}}
\def\AvuT{{A^\transpose_{\vv\vu}}}
\def\BvuT{{B^\transpose_{\vv\vu}}}
\def\AuuInv{{A^{-1}_{\vu\vu}}}
\def\AvvInv{{A^{-1}_{\vv\vv}}}
\def\BuuInv{{B^{-1}_{\vu\vu}}}
\def\BvvInv{{B^{-1}_{\vv\vv}}}
\def\AuuCInv{{\tilde{A}^{-1}_{\vu\vu}}}
\def\BuuCInv{{\tilde{B}^{-1}_{\vu\vu}}}
\def\AvvCInv{{\tilde{A}^{-1}_{\vv\vv}}}
\def\BvvCInv{{\tilde{B}^{-1}_{\vv\vv}}}
\def\AvvInvT{{A^{-\transpose}_{\vv\vv}}}
\def\AuuCInvT{{\tilde{A}^{-\transpose}_{\vu\vu}}}

% \def\Dxu{{\nabla_{\vu \vx}}}
% \def\llxu{{{\ell}(\vx^{(i)},\vu)}}
% \def\ffxu{{{f}(\vx^{(i)},\vu)}}
% \def\Lx{{\mathbf{L}_{\mX}}}
% \def\Lu{{\mathbf{L}_{\vu}}}
% \def\Lxx{{\mathbf{L}_{\mX \mX}}}
% \def\Luu{{\mathbf{L}_{\vu \vu}}}
% \def\Lux{{\mathbf{L}_{\vu \mX}}}
% \def\Fu{{\mathbf{F}_\vu}}
% \def\Fx{{\mathbf{F}_\mX}}
% \def\FxT{{\mathbf{F}_\mX^\transpose}}
% \def\FuT{{\mathbf{F}_\vu^\transpose}}
% \def\Fxx{{\mathbf{F}_{\mX \mX}}}
% \def\Fuu{{\mathbf{F}_{\vu \vu}}}
% \def\Fux{{\mathbf{F}_{\vu \mX}}}
\def\VxN{{\mathbf{V}_\mX^T}}
\def\VxxN{{\mathbf{V}_{\mX\mX}^T}}
% \def\QQX{{\mathbf{Q}_\mX}}
% \def\QQu{{\mathbf{Q}_\vu}}
% \def\QQXX{{\mathbf{Q}_{\mX\mX}}}
% \def\QQuu{{\mathbf{Q}_{\vu\vu}}}
% \def\QQuX{{\mathbf{Q}_{\vu\mX}}}
% \def\QQuuInv{{\mathbf{Q}^{-1}_{\vu\vu}}}
% \def\QQuuInvApprox{{\mathbf{\widetilde{Q}}^{-1}_{\vu\vu}}}
% \def\QQuXT{{\mathbf{Q}^\transpose_{\vu\mX}}}
% \def\VXNxt{{\mathbf{V}^\prime_{\mX}}}
% \def\VXXNxt{{\mathbf{V}^\prime_{\mX\mX}}}

\def\VX{{\mathbf{V}_{\mX}}}
\def\VXX{{\mathbf{V}_{\mX\mX}}}

\def\QQXt{{\mathbf{Q}^t_\mX}}
\def\QQut{{\mathbf{Q}^t_\vu}}
\def\QQXXt{{\mathbf{Q}^t_{\mX\mX}}}
\def\QQuut{{\mathbf{Q}^t_{\vu\vu}}}
\def\QQuXt{{\mathbf{Q}^t_{\vu\mX}}}
\def\QQuuInvt{{[\mathbf{Q}^{t}_{\vu\vu}]^{-1}}}
\def\VXt{{\mathbf{V}^t_{\mX}}}
\def\VXXt{{\mathbf{V}^t_{\mX\mX}}}


\def\xxi{{\vx_t^{(i)}}}

\def\dvx{{\delta\vx}}
\def\dvu{{\delta\vu}}
\def\dvv{{\delta\vv}}
\def\vxTraj{{\bar{\vx}}}
\def\vuTraj{{\bar{\vu}}}

\def\Inv{{-1}}
% \def\Inv{{\dagger}}

\def\ConvT{{\text{ } \hat{*} \text{ }}}
% \def\ConvT{{*^\transpose}}
\def\eqConv{{\text{ }\text{ } \stackrel{\mathclap{\tiny\mbox{conv}}}{=}\text{ }\text{ } }}

\def\Vh{{V_{\vh}}}
\def\Vht{{V^{t}_{\vh}}}
\def\Vhht{{V^{t}_{\vh\vh}}}
% \def\Vxt{{V^{t+1}_{\vx}}}
% \def\Vxxt{{V^{t+1}_{\vx\vx}}}
% \def\Vx{{V_{\vx^{\prime}}^{\prime}}}
% \def\Vxx{{V_{\vx^{\prime} \vx^{\prime}}^{\prime}}}

% \def\Qxt{{Q^t_{\vx}}}
% \def\Qut{{Q^t_{\vu}}}
% \def\Qxxt{{Q^t_{\vx \vx}}}
% \def\Quxt{{Q^t_{\vu \vx}}}
% \def\Qxut{{Q^t_{\vx \vu}}}
% \def\Quut{{Q^t_{\vu \vu}}}
% \def\Qx{{Q_{\vx}}}
% \def\Qu{{Q_{\vu}}}
% \def\Qxx{{Q_{\vx \vx}}}
% \def\Quu{{Q_{\vu \vu}}}
% \def\QuuInv{{Q^{-1}_{\vu \vu}}}
% \def\QuuInvt{{({Q^{t}_{\vu \vu})}^{-1}}}
% \def\Qux{{Q_{\vu \vx}}}
% \def\Qxu{{Q_{\vx \vu}}}

% \def\Qvt{{Q^t_{\vv}}}
% \def\Qvxt{{Q^t_{\vv \vx}}}
% \def\Qvyt{{Q^t_{\vv \vx_r}}}
% \def\Qxvt{{Q^t_{\vx \vv}}}
% \def\Qvvt{{Q^t_{\vv \vv}}}
% \def\Quvt{{Q^t_{\vu \vv}}}
% \def\Qvut{{Q^t_{\vv \vu}}}
% \def\Qv{{Q_{\vv}}}
% \def\Qvv{{Q_{\vv \vv}}}
% \def\QvvInv{{Q^{-1}_{\vv \vv}}}
% \def\QvvInvt{{({Q^{t}_{\vv \vv})}^{-1}}}
% \def\Qvx{{Q_{\vv \vx}}}
% \def\Qxv{{Q_{\vx \vv}}}
% \def\Quv{{Q_{\vu \vv}}}
% \def\Qvu{{Q_{\vv \vu}}}
% \def\Qvy{{Q_{\vv \vx_r}}}
% \def\QvuT{{Q^\transpose_{\vv \vu}}}

\def\fx{{{f}_{\vx}}}
\def\fu{{{f}_{\vu}}}
\def\fxt{{{f}^t_{\vx}}}
\def\fut{{{f}^t_{\vu}}}
\def\fuT{{{f}_{\vu}^\transpose}}
\def\fxT{{{f}_{\vx}^\transpose}}
\def\futT{{{{f}^t_{\vu}}^\transpose}}
\def\fxtT{{{{f}^t_{\vx}}^\transpose}}
\def\fxx{{{f}_{\vx \vx}}}
\def\fuu{{{f}_{\vu \vu}}}
\def\fux{{{f}_{\vu \vx}}}
\def\fxu{{{f}_{\vx \vu}}}
\def\fxxt{{{f}^t_{\vx \vx}}}
\def\fuut{{{f}^t_{\vu \vu}}}
\def\fuxt{{{f}^t_{\vu \vx}}}
\def\fxut{{{f}^t_{\vx \vu}}}

\def\gutT{{{g}^{t \text{ }\transpose}_{\vu}}}
\def\gxtT{{{g}^{t \text{ }\transpose}_{\vx}}}
\def\gut{{{g}^{t}_{\vu}}}
\def\gxt{{{g}^{t}_{\vx}}}
\def\sht{{{\sigma}^{t}_{\vh}}}
\def\shtT{{{\sigma}^{t \text{ }\transpose}_{\vh}}}

\def\lxt{{{\ell}^t_{\vx}}}
\def\lut{{{\ell}^t_{\vu}}}
\def\lxxt{{{\ell}^t_{\vx \vx}}}
\def\luut{{{\ell}^t_{\vu \vu}}}
\def\luxt{{{\ell}^t_{\vu \vx}}}
\def\lxut{{{\ell}^t_{\vx \vu}}}


\def\lx{{{\ell}_{\vx}}}
\def\lu{{{\ell}_{\vu}}}
\def\lxx{{{\ell}_{\vx \vx}}}
\def\luu{{{\ell}_{\vu \vu}}}
\def\lux{{{\ell}_{\vu \vx}}}
\def\lxu{{{\ell}_{\vx \vu}}}

\def\gx{{{g}_{\vx}}}
\def\gu{{{g}_{\vu}}}
\def\gxx{{{g}_{\vx \vx}}}
\def\guu{{{g}_{\vu \vu}}}
\def\gux{{{g}_{\vu \vx}}}
\def\gxu{{{g}_{\vx \vu}}}

\def\gxxt{{{g}^t_{\vx \vx}}}
\def\guut{{{g}^t_{\vu \vu}}}
\def\guxt{{{g}^t_{\vu \vx}}}
\def\gxut{{{g}^t_{\vx \vu}}}


\def\Dxu{{\nabla_{\vu \vx}}}
\def\llxu{{{\ell}(\vx^{(i)},\vu)}}
\def\ffxu{{{f}(\vx^{(i)},\vu)}}
% \def\Lx{{\mathbf{L}_{\mX}^t}}
% \def\Lu{{\mathbf{L}_{\vu}^t}}
% \def\Lxx{{\mathbf{L}^t_{\mX \mX}}}
% \def\Luu{{\mathbf{L}^t_{\vu \vu}}}
% \def\Lux{{\mathbf{L}^t_{\vu \mX}}}

% \def\Fu{{\mathbf{F}^t_\vu}}
% \def\Fx{{\mathbf{F}^t_\mX}}
% \def\FxT{{{\mathbf{F}^{t\transpose}_\mX}}}
% \def\FuT{{{\mathbf{F}^{t\transpose}_\vu}}}
% \def\Fxx{{\mathbf{F}^t_{\mX \mX}}}
% \def\Fuu{{\mathbf{F}^t_{\vu \vu}}}
% \def\Fux{{\mathbf{F}^t_{\vu \mX}}}

% \def\Gu{{\mathbf{G}^t_\vu}}
% \def\Gx{{\mathbf{G}^t_\mX}}
% \def\GxT{{{\mathbf{G}^{t\transpose}_\mX}}}
% \def\GuT{{{\mathbf{G}^{t\transpose}_\vu}}}
% \def\Gxx{{\mathbf{G}^t_{\mX \mX}}}
% \def\Guu{{\mathbf{G}^t_{\vu \vu}}}
% \def\Gux{{\mathbf{G}^t_{\vu \mX}}}

\def\VH{{\mathbf{V}^t_{\mH}}}
\def\VhN{{\mathbf{V}_\mH^T}}
\def\VhhN{{\mathbf{V}_{\mH\mH}^T}}
\def\VHNxt{{\mathbf{V}^\prime_{\mH^\prime}}}
\def\VHHNxt{{\mathbf{V}^t_{\mH\mH}}}


% \def\VxN{{\mathbf{V}_\mX^T}}
% \def\VxxN{{\mathbf{V}_{\mX\mX}^T}}
\def\QQX{{\mathbf{Q}_\mX^t}}
\def\QQu{{\mathbf{Q}_\vu^t}}
\def\QQXX{{\mathbf{Q}^t_{\mX\mX}}}
\def\QQuu{{\mathbf{Q}^t_{\vu\vu}}}
\def\QQuX{{\mathbf{Q}^t_{\vu\mX}}}
\def\QQuuInv{{\mathbf{Q}^{-1}_{\vu\vu}}}
\def\QQuuInvApprox{{\mathbf{\widetilde{Q}}^{-1}_{\vu\vu}}}
\def\QQuXT{{{\mathbf{Q}^{t\transpose}_{\vu\mX}}}}
\def\VXNxt{{\mathbf{V}^\prime_{\mX^\prime}}}
\def\VXXNxt{{\mathbf{V}^\prime_{\mX^\prime\mX^\prime}}}

\def\QQXprevT{{\mathbf{Q}_\mX^{T-1}}}
\def\QQuprevT{{\mathbf{Q}_\vu^{T-1}}}
\def\QQXXprevT{{\mathbf{Q}^{T-1}_{\mX\mX}}}
\def\QQuuprevT{{\mathbf{Q}^{T-1}_{\vu\vu}}}
\def\QQuXprevT{{\mathbf{Q}^{T-1}_{\vu\mX}}}

\def\VX{{\mathbf{V}_{\mX}}}
\def\VXX{{\mathbf{V}_{\mX\mX}}}

\def\QQXt{{\mathbf{Q}^t_\mX}}
\def\QQut{{\mathbf{Q}^t_\vu}}
\def\QQXXt{{\mathbf{Q}^t_{\mX\mX}}}
\def\QQuut{{\mathbf{Q}^t_{\vu\vu}}}
\def\QQuXt{{\mathbf{Q}^t_{\vu\mX}}}
\def\QQuuInvt{{(\mathbf{Q}^{t}_{\vu\vu})^{-1}}}
\def\VXt{{\mathbf{V}^t_{\mX}}}
\def\VXXt{{\mathbf{V}^t_{\mX\mX}}}

\def\idxFu{{(B_{n_{t^\prime}}^{(i)},:)}}
\def\idxFuu{{(B_{n_{t^\prime}}^{(i)},:,:)}}
\def\idxFx{{(B_{n_{t^\prime}}^{(i)},B_{n_{t}}^{(j)})}}
\def\idxFux{{(B_{n_{t^\prime}}^{(i)},:,B_{n_{t}}^{(j)})}}
\def\idxFxx{{(B_{n_{t^\prime}}^{(i)},B_{n_{t}}^{(j)},B_{n_{t}}^{(k)})}}

%%%%%%%%%%%%%%%%%%%%%%%%%%
% Mean field optimal control
%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\cspace{{\mathbb{R}^{m}}}
\def\Cspace{{\mathbb{R}^{\bar{m}}}}
\def\Xspace{{\mathbb{R}^{n}}}
\def\xyspace{{\mathbb{R}^{n+d}}}
% \def\Cspace{{\mathbb{R}^{mT}}}
\def\yspace{{\mathbb{R}^{d}}}
\def\expdnn{{\mathbb{E}_{\substack{ (\rvx_t, \rvy) \sim \mu_t \\ \text{subject to (\ref{eq:fc-dnn-dynamics})}}}}}% expectation

\def\transpose{{\mathsf{T}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%
% SGD formulation
%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\gradsampleeq{{
    \nabla_\vtheta l ( f ( \rvx^{(i)}, \vtheta ), \rvy^{(i)} )
}}
\def\gradsample{{ g^{i}(\vtheta) }}
\def\gradmb{{ g^{mb}(\vtheta) }}
\def\gradfull{{ g^{}(\vtheta) }}
\def\gradmbt{{   g^{mb}(\vtheta_{t}) }}
\def\gradfullt{{ g^{}(\vtheta_{t}) }}
\def\diffusionmatrixx{{ \mathbf{\Sigma}_{\mathcal{D}} }}
\def\diffusionmatrix{{ \mathbf{\Sigma}_{\mathcal{D}}(\vtheta) }}
\def\diffusionmatrixt{{ \mathbf{\Sigma}_{\mathcal{D}}(\vtheta_{t}) }}
% \def\diffusionmatrixthaft{{  \mathbf{\Sigma}^{1/2}_{        \mathcal{D}}(\vtheta_{t}) }}
\def\diffusionmatrixthaft{{ \mathbf{\Sigma}^{\frac{1}{2}}_{\mathcal{D}}(\vtheta_{t}) }}
\def\diffusionmatrixthaftt{{ \mathbf{\Sigma}^{\frac{1}{2}}_{\mathcal{D}} }}
% \def\diffusionmatrixthafttt{{ \tilde{\mathbf{\Sigma}}^{\frac{1}{2}}_{\mathcal{D}}(\vtheta_{t}) }}
\def\diffusionmatrixthafttt{{ \tilde{\mathbf{\Sigma}}^{\frac{1}{2}}_{\mathcal{D}} }}
\def\diffusionmatrixttt{{ \tilde{\mathbf{\Sigma}}_{\mathcal{D}} }}
\def\diffusionmatrixbatch{{ \tilde{\mathbf{\Sigma}}_{\mathcal{B}} }}
%
% \def\abs#1{ \mid {#1} \mid }
\def\absB{{ \mid \mathcal{B} \mid }}
\def\absD{{ \mid \mathcal{D} \mid }}
%
\def\drift{{ b(\vtheta_{t}) }}
\def\diffusion{{ \sigma(\vtheta_{t}) }}
\def\dt{{ \mathrm{d} t }}
\def\ds{{ \mathrm{d} s }}
\def\dWt{{ \mathrm{d} \mathbf{W}_t }}
\def\dLat{{ \mathrm{d} L_t^{\alpha} }}
\def\tt{{ \vtheta_{t} }}

\def\pss{{ \rho^{\mathrm{ss}} }}
\def\psss{{ \rho^{\mathrm{ss}}(\vtheta) }}

\def\Dk{{ \mathrm{D}^k }}
\def\gmbupdate{{ \vtheta^{\prime} - \eta g^{mb}(\vtheta^{\prime}) }}
\def\gmbupdatee{{ \vtheta - \eta g^{mb}(\vtheta) }}
% \def\deltaa{{ \delta\left( \vtheta - \left(\gmbupdate\right) \right) }}
\def\deltaa{{ \delta\left\{ \vtheta - \left[\gmbupdate\right] \right\} }}
\def\thprime{{ \vtheta^{\prime} }}
\def\dthprime{{ \mathrm{d} \thprime }}
\def\dth{{ \mathrm{d} \vtheta }}
\def\expB{{   \mathbb{E}_{\mathcal{B}} }}
\def\expPss{{ \mathbb{E}_{\pss} }}
% \def\smallint{\begingroup\textstyle \int\endgroup}
\def\smallint{ \int}
\def\smallsum{\begingroup\textstyle \sum \endgroup}

\def\expBof#1{ \expB \left[ {#1} \right]}
\def\expPssof#1{ \expPss \left[ {#1} \right]}
\def\Phigmd{{ \Phi \left(\gmbupdatee\right) }}

\def\itoarg{{\left( X_t, t \right) }}


%%%%%%%%%%%%%%%%%%%%%%%%%%
% Beyong Supervised Learning
%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\thetap{{ \vtheta^{\prime} }}
\def\LocalEntropy{{ - \log \int_{\thetap \in \cspace} \exp (-\Phi (\thetap)-\frac{\gamma}{2}\|\vtheta-\thetap\|_{2}^{2}) \mathrm{d} \thetap }}
\def\LocalEntropyy{{ - \log \int_{\thetap} \exp \left(-\Phi (\thetap)-\frac{\gamma}{2}\|\vtheta-\thetap\|_{2}^{2}\right) \mathrm{d} \thetap }}
\def\ExpOf#1{ \mathbb{E} \left[ {#1} \right]}
\def\ExpOfXi#1{ \mathbb{E}_\xi \left[ {#1} \right]}
\def\ExpOfGibbs#1{ \mathbb{E}_{ \mathcal{P}_\gamma} \left[ {#1} \right]}
\def\fracK {{\frac{1}{k}}}

\def\metanext{{ \vtheta_{\text{adapt}}^{n+1} }}
\def\metacurr{{ \vtheta_{\text{adapt}}^{n}   }}


%Capital caligraphic letters
\def\calA{{\cal A}}
\def\calB{{\cal B}}
\def\calC{{\cal C}}
\def\calD{{\cal D}}
\def\calE{{\cal E}}
\def\calF{{\cal F}}
\def\calG{{\cal G}}
\def\calH{{\cal H}}
\def\calI{{\cal I}}
\def\calJ{{\cal J}}
\def\calK{{\cal K}}
\def\calL{{\cal L}}
\def\calM{{\cal M}}
\def\calN{{\cal N}}
\def\calO{{\cal O}}
\def\calP{{\cal P}}
\def\calQ{{\cal Q}}
\def\calR{{\cal R}}
\def\calS{{\cal S}}
\def\calT{{\cal T}}
\def\calU{{\cal U}}
\def\calV{{\cal V}}
\def\calW{{\cal W}}
\def\calX{{\cal X}}
\def\calY{{\cal Y}}
\def\calZ{{\cal Z}}

\newcommand{\nicefracpartial}[2]{\nicefrac{\partial #1}{\partial  #2}}
\newcommand{\nicefracdiff}[2]{\nicefrac{\rd #1}{\rd  #2}}
\newcommand{\fracpartial}[2]{\frac{\partial #1}{\partial  #2}}
\newcommand{\fracdiff}[2]{\frac{\rd #1}{\rd  #2}}
\newcommand{\br}[1]{\left[#1\right]}
\newcommand{\pr}[1]{\left(#1\right)}
\newcommand{\T}{\mathsf{T}}
\newcommand*\bvec[1]{\begin{bmatrix}#1\end{bmatrix}}
\newcommand{\bmat}[4]{\begin{bmatrix} #1 & #2 \\ #3 & #4\end{bmatrix}}
\def\vec{{\mathrm{vec}}}

